Reactive Temporal Logic-based Planning and Control for Interactive Robotic Tasks

Robots interacting with humans must be safe, reactive and adapt online to unforeseen environmental and task changes. Achieving these requirements concurrently is a challenge as interactive planners lack formal safety guarantees, while safe motion planners lack flexibility to adapt. To tackle this, we propose a modular control architecture that generates both safe and reactive motion plans for human-robot interaction by integrating temporal logic-based discrete task level plans with continuous Dynamical System (DS)-based motion plans. We formulate a reactive temporal logic formula that enables users to define task specifications through structured language, and propose a planning algorithm at the task level that generates a sequence of desired robot behaviors while being adaptive to environmental changes. At the motion level, we incorporate control Lyapunov functions and control barrier functions to compute stable and safe continuous motion plans for two types of robot behaviors: (i) complex, possibly periodic motions given by autonomous DS and (ii) time-critical tasks specified by Signal Temporal Logic~(STL). Our methodology is demonstrated on the Franka robot arm performing wiping tasks on a whiteboard and a mannequin that is compliant to human interactions and adaptive to environmental changes.

==> Controllable_prop.tex <==
We introduce a generalized version of the predicates~$\mu$ described in~\ref{sec:stl} as controllable propositions.
\begin{definition}
The truth value of a controllable proposition~$p_c$ is defined below using a tuple $\left(\mathcal{L}, \mathcal{M}, \mathfrak{U}\right)$, where ${\mathcal{L} : \mathbb{R}^d \to \mathfrak{U}}$, ${\mathcal{M}: \mathbb{R}^d \to 2^{\mathfrak{U}}}$, and $2^{\mathfrak{U}}$ is the power set of $\mathfrak{U}$.
\begin{equation}
p_c = \begin{cases}
    true & \Leftrightarrow \mathcal{L}(x(t)) \in \mathcal{M}(x(t))\\
    false & \Leftrightarrow \mathcal{L}(x(t)) \notin \mathcal{M}(x(t))
\end{cases}
    \label{control_prop_eqn}
\end{equation}
    \label{control_prop_def}
\end{definition}
\change{there exists a control $u$ such that $p_c$ is true?}
The predicates~$\mu$ that define STL tasks in Section~\ref{sec:stl} is a controllable proposition where ${\mathfrak{U}=\mathbb{R}, \mathcal{L}(x(t)) = h(x(t))}$ and ${\mathcal{M}(x(t)) =  \mathbb{R}_{\geq 0}}$ for all $x(t) \in \mathbb{R}^d$. We also interpret a nominal autonomous dynamical system~${\dot{x} = d_i(x)}$ for each motion~$i$ described in Section~\ref{sec:LfD_prelim} as a controllable proposition, where $\mathfrak{U}=\mathbb{R}^d, \mathcal{L}(x(t)) = \dot{x}(t)$ and ${\mathcal{M}(x(t)) =  \{d_i(x(t))\}}$. We switch between different DS based motions~$d_i(x)$ online at task execution which correspond to satisfying different controllable propositions at each time step. For example, the behavior of \textit{stir every 10 secs} in Example~\ref{pasta_cooking_example} could correspond to executing a DS based motion for stirring and being stationary ($\dot{x}(t) = 0$) for 10 seconds. We denote the propositions $p_c$ in Definition~\ref{control_prop_def} as \textit{controllable} because their truth value entirely depends on the robot's state $x(t)$ which can be controlled by $u$ in~\eqref{nonlinear_DS}. The syntax of a temporal logic built using $p_c$ as the building block is

==> Related_work.tex <==
\section{Related work}
\label{sec:realted_work}

\subsection{Learning from Demonstrations}
\label{sec:LfD_related}

Behaviour Cloning (BC) and Inverse Reinforcement Learning (IRL)~\cite{abbeel2004apprenticeship, BC, IOC} are popular LfD approaches that accurately reproduce complex tasks, but typically require large amounts of data and also explore the state space, which is not feasible when the demonstrator is a human. Popular imitation algorithms such as DAgger~\cite{DAGGER} and deep imitation learning~\cite{deep_imit} are also data-hungry, and further provide no stability or safety guarantees. We base our approach on Dynamical System (DS) based motion planning approches~\cite{figueroa2018physically, billard2022learning, SO3_1, multi_arm} that learn a global vector field instead of discrete way-points. Existing DS based LfD approaches have shown to reproduce stable motions using very few demonstrations (3-4) that are both reactive and compliant to external perturbations, which are necessary for physical human-robot interactions online. In our previous work~\cite{nawaz2023learning}, we propose a DS based method utilizing a Neural ODE~\cite{chen2018neural} to learn intricate periodic motions such as wiping and stirring, from just 3-4 demonstrations. Our method ensures robustness to online disturbances and unforeseen obstacles through the incorporation of Control CLF and CBF, respectively.

\subsection{Formal methods for control synthesis}
\label{sec:formal_methods}

Inspired from the literature of hybrid systems~\cite{discrete_hybrid, languages_hybrid}, a variety of approaches have enabled the formal integration of high-level discrete actions to low-level continuous motion plans~\cite{integrated, hybrid}. Researchers have used formal methods for control synthesis~\cite{formal_control} to solve the complete planning problem, where the generated controllers satisfy high-level specifications described using LTL~\cite{principles_model_check, nawaz2020explorative} or STL~\cite{robust_STL}. LTL has been widely used to capture discrete events~\cite{LTL_multi, farhad_LTL}, while STL can capture continuous timing constraints~\cite{STL_timing} for complex tasks. Prior work using temporal logic either lacks responsiveness to online events and disturbances~\cite{jones2019scratchs} or depends on computationally intensive mixed-integer linear programs~\cite{raman2015reactive, SMT} for online adaptation and robustness against disturbances. Generalized Reactivity~(1) formula~\cite{GR1, temporal_imit} is a framework for reactive motion planning that relies on a discrete abstraction of the state space which results in a large computation burden for planning. We formulate our motion planner as a Quadratic Program~(QP) with the incorporation of CLFs and CBFs~\cite{ames2019control, stl_lars}. This approach ensures computational efficiency while maintaining the continuous state space model for low-level planning. Simultaneously, our task planner employs LTL for discrete reasoning in handling reactive tasks.



==> STL_CBF.tex <==
\section{Task Planner
Given a task specification $\Psi$, we construct the corresponding B\"uchi automaton ${\mathcal{B}_{\Psi}= (\mathcal{S}, s_0, AP, \delta, \mathcal{F})}$ using Spot~2.0~\cite{spot_2}. We denote $s$ to be the current state of the automaton, $\sigma_c$ and $\sigma_u$ to be the controllable and uncontrollable propositions that are \textit{true} at the given time step. We first initialize the relevant variables. At each time step, the task planner receives $[\sigma_c, \sigma_u]$ as an input. If there is a change in the values of the uncontrollable propositions, we modify the directed graph $\mathcal{G}(\mathcal{S}, E) \gets \textrm{Graph}(\mathcal{B}_{\Psi}, \sigma_u)$ by removing the transitions that violate the current value of uncontrollable propositions $\sigma_u$, i.e., for all $s_1, s_2 \in \mathcal{S}$,
\begin{alignat*}{1}
    &(s_1, s_2) \in E \Leftrightarrow \exists p_c \in \mathcal{A}_c \ \textrm{s.t.} \ \delta(s_1, [p_c, \sigma_u]) = s_2
\end{alignat*}
Then, we plan a shortest path using breadth first search~\cite{BFS} that reaches an accepting state in $\mathcal{F}$ and visits $\mathcal{F}$ infinitely often. The obtained path:=$\{s_0, s_1, s_2, \ldots\}$, where ${\inf\left(\textrm{path}\right) \cap \mathcal{F} \neq \emptyset, \ s_0 = s, \ \delta(s_i, [\sigma_c^i, \sigma_u]) = s_{i+1}}$ for all $i \geq 0$ and $\sigma_c^i \in \mathcal{A}_c$ is the controllable proposition that has to be true when transition from $s_i$ to $s_{i+1}$. Such a path generates a sequence of transitions on $\mathcal{B}_{\Psi}$ that satisfies $\Psi$~\cite{event_STL}. Since we consider formulas of the form~\eqref{reactive_TL_syntax} and compute the shortest path for a fixed realisation of uncontrollable propositions $\sigma_u$, the choice of shortest paths will entirely depend on the controllable proposition that is true in each transition as described in~\cite{event_STL}. Specifically, under Assumption~\ref{assum_1} and the syntax~\eqref{reactive_TL_syntax}, the label of each transition in the graph $\mathcal{G}$ is given by 
\begin{equation}
l := \lor_{i=1}^K \left(U_i \land V_i\right),
    \label{label_form}
\end{equation}
where $\sigma_u \vDash U_i$ and $V_i \in \mathcal{A}_c$ for all $i \in \{1,2,\ldots,K\}$. The outgoing transition from the current state $s$ along the shortest path is given by current\_transition. If there is an external environmental event that changes the value of uncontrollable propositions, lines 2-5 in Algorithm~\ref{alg:task_plan} are implemented to plan a shortest path on the modified graph. Otherwise, lines 7-11 are implemented to move along the current shortest path. Then, we update the automaton states and propositions in line 13. In line 14, we choose the type of motion plan $\sigma_m$ based on current\_transition. Each transition has a label of the form~\eqref{label_form} and we choose $\sigma_{m} = C_i$ such that $U_i = true$. If there are multiple such $C_i$, then we choose them at random since any of them will transition along the shortest path to the accepting states. However, we observed from our experience that the transitions will have exactly one~$C_i$ for each unique~$U_i$. 

For example, the automaton $\mathcal{B}_{\Psi}$ is given in Fig.~\ref{fig:aut_eg_small} for the same specification ${\Psi := G (\textit{h} \Rightarrow \textit{s}) \land G (\neg \textit{h} \Rightarrow F \textit{(p)})}$ described in Section~\ref{sec:reactive_TL}, where ${h := hot, \ s:=stir, \ p:=press \ button}$. If the initialisation is such that $s=0, h = 1, s = 1, p = 0$, then the shortest path is just the self transition $0 \to 0$. Then, from the label of the transition $0 \to 0$ and $\sigma_u = \{h\}$, the motion plan to be implemented is $\sigma_m = s$ so that the robot follows the behavior \textit{stir}. If $h=0$ while the robot is stirring, then the system transitions to state $1$. Now, the shortest path is computed again and the path is $1 \to 0 \to 0$. From the label of the transitions $1 \to 0 \to 0$ and $h = 0$, the motion plan to be implemented is $\sigma_m = p$ so that the robot follows the behavior \textit{press button}. In the next section, we describe how the desired behavior $\sigma_m$ is achieved by implementing a DS-based motion plan.  
% \begin{wrapfigure}{R}{0.5\textwidth}
\RestyleAlgo{ruled}
\LinesNumbered
%% This is needed if you want to add comments in
%% your algorithm with \Comment
% \SetKwComment{Comment}{/* }{ */}
\setlength{\textfloatsep}{0pt}% Remove \textfloatsep
% \addtocounter{algocf}{1}
\begin{algorithm}[!h]
\caption{Task Planner}
\label{alg:task_plan}
\KwInit{\\
$\mathcal{B}_{\Psi}:=(\mathcal{S}, s_0, \mathcal{A}_c \cup \mathcal{A}_u, \delta, \mathcal{F}) \gets \textrm{Automaton}(\Psi)$\\
$s', [\sigma_c', \sigma_u']$ where $s' \in \mathcal{S}, \sigma_c' \in \mathcal{A}_c, \sigma_u' \subseteq \mathcal{A}_u$\\
$\mathcal{G}(\mathcal{S}, E) \gets \textrm{Graph}(\mathcal{B}_{\Psi}, \sigma_u')$ \\
 $\textrm{path} \gets \textrm{ShortestPath}(\mathcal{G}, s', \mathcal{F})$\;
}
\KwInput{$\ [\sigma_c, \sigma_u]$ where $\sigma_c \in \mathcal{A}_c, \sigma_u \subseteq \mathcal{A}_u$}
\KwResult{Type of motion plan to implement $\sigma_{m}$}
\eIf{$\sigma_u \neq \sigma_u'$}{
  $\mathcal{G}(\mathcal{S}, E) \gets \textrm{Graph}(\mathcal{B}_{\Psi}, \sigma_u)$\;
    $s \gets \delta(s', [\sigma_c, \sigma_u])$\;
    $\textrm{path} \gets \textrm{ShortestPath}(\mathcal{G}, s, \mathcal{F})$\;
    $\textrm{current\_transition} \gets \textrm{path.transition}$\;
  }{
  $s \gets \delta(s', [\sigma_c, \sigma_u])$\;
  \If{$s \neq s'$}{
      $\textrm{path} \gets \textrm{path.next}$\;
    }
$\textrm{current\_transition} \gets \textrm{path.transition}$\;
  }
  $s' \gets s, \ \sigma_c' \gets \sigma_c, \sigma_u' \gets \sigma_u$\;
  $\sigma_{m} \gets \textrm{MotionPlan}(\textrm{current\_transition})$ \change{Another algorithm to describe this function?}\;
  \end{algorithm}}

\section{Reactive TL semantics}

\begin{alignat*}{5}
&(x, \sigma, t) &&\vDash \psi &&\Leftrightarrow&&(x, t) \vDash \psi \\
&(x, \sigma, t) &&\vDash G (\varphi \Rightarrow \Psi) &&\Leftrightarrow&&  (\sigma, t) \nvDash \varphi \ \textrm{or} \\
& && && && \left((\sigma, t) \vDash \varphi \ \textrm{and} \ (x, \sigma, t) \vDash \Psi\right) \\
&(x, \sigma, t) &&\vDash G (\Psi_1 \Rightarrow \Psi_2) &&\Leftrightarrow&&  (x, \sigma, t) \nvDash \Psi_1 \textrm{or} \\
& && && &&\left((x, \sigma, t) \vDash \Psi_1 \ \textrm{and} \ (x, \sigma, t) \vDash \Psi_2\right) \\
&(x, \sigma, t) &&\vDash \Psi_1 \land \Psi_2  &&\Leftrightarrow&&  (x, \sigma, t) \vDash \Psi_1 \ \textnormal{and} \ (x, \sigma, t) \vDash \Psi_2 
\label{rtl_semantics}
\end{alignat*}

\section{CTL syntax semantics}

Consider a finite set of controllable propositions $\mathcal{A}_c$, where each $p_c \in \mathcal{A}_c$ can either be \textit{true} or \textit{false} as defined by~\ref{control_prop_eqn}. A Controllable Temporal Logic~(CTL) formula $\phi$ is constructed over~$\mathcal{A}_c$ using the following syntax.
\begin{equation}
\varphi ::= \textit{true} \ | \ p_c \ | \ \neg \phi \ | \ \phi_1 \land \phi_2 \ | \ \phi_1 U \phi_2 
    \label{ltl_form}
\end{equation}
The semantics of CTL are defined below, where $(x, t) \vDash \phi$ indicates that the state signal $x : \mathbb{R}_{\geq 0} \to \mathbb{R}^d$ satisfies a formula $\phi$ at time $t$. 
\begin{alignat*}{5}
&(x, t) &&\vDash true &&\Leftrightarrow&& \textnormal{holds by definition} \\
&(x, t) &&\vDash p_c &&\Leftrightarrow&&  \mathcal{L}(x(t)) \in \mathcal{M}(x(t)) \\
&(x, t) &&\vDash \neg \phi  &&\Leftrightarrow&&  (x, t) \nvDash \phi \\
&(x, t) &&\vDash \varphi_1 \land \varphi_2  &&\Leftrightarrow&&  (x, t) \vDash \phi_1 \ \textnormal{and} \ (x, t) \vDash \varphi_2 \\
&(x, t) &&\vDash \phi_1 U \phi_2  &&\Leftrightarrow&&  \exists t'' \geq t \ \textnormal{s.t.} \ (x, t'') \vDash \phi_2 \ \textnormal{and} \\
& && && &&\forall \ t' \in [t, t''), \ (x, t') \vDash \phi_1 \\
&(x, t) &&\vDash F \varphi  &&\Leftrightarrow&&  \exists t' \geq t \ \textnormal{s.t.} \ (x, t') \vDash \phi \\
&(x, t) &&\vDash G \varphi  &&\Leftrightarrow&&  \forall t' \geq t, \ (x, t') \vDash \varphi 
\label{ctl_semantics}
\end{alignat*}

\section{STL prelims}

The syntax for the STL formula $\phi$ is given as
\begin{equation}
\phi ::= \textit{true} \ | \ \mu \ | \ \neg \phi \ | \ \phi_1 \land \phi_2 \ | \ \phi_1 U_I \phi_2
    \label{stl_form}
\end{equation}
Notice the time interval $I$ in all the temporal operators in~\eqref{stl_form} which will be used for time-critical tasks. 

For a given state signal $x : \mathbb{R}_{\geq 0} \to \mathbb{R}^d$, where $d$ is the dimension of the state space, the semantics of the STL formula are given below.
\begin{alignat*}{7}
&(x, t) &&\vDash true &&\Leftrightarrow&& \textnormal{holds by definition} \\
&(x, t) &&\vDash \mu &&\Leftrightarrow&& h(x(t)) \geq 0 \\
&(x, t) &&\vDash \neg \phi  &&\Leftrightarrow&&  (x, t) \nvDash \phi \\
&(x, t)  &&\vDash \phi_1 \land \phi_2  &&\Leftrightarrow&&  (x, t) \vDash \phi_1 \ \textnormal{and} \ (x, t) \vDash \phi_2 \\
&(x, t) &&\vDash \phi_1 U_I \phi_2  &&\Leftrightarrow&&  \exists t'' \in t \oplus I \ \textnormal{s.t.} \ (x, t'') \vDash \phi_2 \ \textnormal{and} \\
& && && &&\forall \ t' \in [t, t''), \ (x, t') \vDash \phi_1 \\
&(x, t) &&\vDash F_I \phi  &&\Leftrightarrow&&  \exists t' \in t \oplus I \ \textnormal{s.t.} \ (x, t') \vDash \phi \\
&(x, t) &&\vDash G_I \varphi  &&\Leftrightarrow&&  \forall t' \in t \oplus I, \ (x, t') \vDash \phi 
     \label{stl_semantics}
\end{alignat*}
